Effects of sweeps and ejections on amplitude modulation in a turbulent channel flow

Conditional averages are used to evaluate the effect of sweeps and ejections on amplitude modulation. This is done numerically with a direct numerical simulation (DNS) of a channel flow at friction Reynolds number $Re_{\tau} = 1000$ in a minimal stream-wise unit (MSU). The amplitude-modulation map of such DNS is also compared to the one of a regular channel flow in a longer streamwise domain (LSD), in order to assess its validity for this study. The cheaper MSU is found to provide a good representation of the modulation phenomena in the LSD. As for conditional averages, the amplitude-modulation coefficient is conditioned on the sign of the large-scale fluctuations. Care must be exerted in defining such a coefficient, as the conditioned large-scale fluctuation has non-zero average, indeed as a consequence of conditioning. Both sweeps and ejections (positive and negative large-scale fluctuation events) are found to have a positive contribution to amplitude modulation in the buffer layer, and a negative one in the outer layer. The negative-modulation region is found to shrink in case of ejections, so that the positive-modulation region extends farther away from the wall. Two more conditional statistics are used to provide an alternative representation of amplitude modulation and insights into the characteristics of the large-scale structures.

==> tab/numpar.tex <==
\begin{table}
\begin{tabular*}{1.0\textwidth}{@{\extracolsep{\fill}} l c c c c c c c c c c c}
Type & $Re_\tau$ & $Re_b$ & $L_x/h$& $L_z/h$ & $L_x^+$& $L_z^+$& $N_x \times N_y \times N_z$ & $\Delta x^+$ & $\Delta z^+$ & $\Delta y^+_{\mathrm{min}}$ & $T u_\tau/h $\\[10pt]

LSD       & 1000 & 19995  & $4\pi$    & $2\pi$    & 12566   & 6283   & $1024\times  500 \times 1024$ & 12.3 & 6.1 & XXX & XXX\\
MSU       & 1000 & 20758  & 0.4       & 7         &   400   & 7000   & $  40 \times 500 \times 1148$ & 10.0 & 6.1 & XXX & XXX	
\end{tabular*}
\caption{Details of the Long Streamwise Domain (LSD) and Minimal Streamwise Unit (MSU) simulations. $Re_b$ and $Re_\tau$ are respectively the bulk and friction Reynolds number, $L_x$ and $L_z$ are the streamwise and spanwise extent of the computational box, $N_x$ and $N_z$ are the numbers of Fourier modes in the homogeneous directions (additional modes are used for dealiasing, according to the 3/2 rule), while $N_y$ is the number of collocation points in the wall-normal direction. The resulting spatial resolution is also reported. $T$ is the temporal interval over which statistics have been collected. }
\label{tab:discretization-parameters}
\end{table}

